Surface Melting and Breakup of Metal Nanowires: Theory and Molecular Dynamics Simulations

We consider the surface melting of metal nanowires by solving a phenomenological two-parabola Landau model and by conducting molecular dynamics simulations of nickel and aluminium nanowires. The model suggests that surface melting will precede bulk melting when the spreading parameter $\Delta \gamma$ for the melt in contact with the solid surface is positive (i.e. if the melt wets or partially wets the surface) and the wire is sufficiently thick, as is the case for planar surfaces and sufficiently large nanoparticles. Surface melting does not occur if $\Delta \gamma$ is negative. We test this model, which assumes the surface energies of the wire are isotropic, using molecular dynamics simulations. For nickel, we observe the onset of anisotropic surface melting associated with each of the two surface facets present, but this gives way to uniform surface melting and the solid melts radially until the solid core eventually breaks up. For aluminium, while we observe complete surface melting of one facet, the lowest energy surface remains partially dry even up to the point where the melt completely penetrates the solid core.

==> Free_Eng.tex <==
% \section{Phenomenological model}\label{S: F_eval}
\section{Free energy evaluation of surface and linear melting}
\label{SS: F_surf_lin}

In this section we extend the simple phenomenological model for surface melting that was presented in Section~\ref{S: F_eval} in order to describe the break up of the solid wire seen in the molecular dynamics simulations. The simple geometry in this model is the same as that used in Section~\ref{S: F_eval}, but we now introduce the possibility of a liquid gap of width $h$ initiating the break up of the solid portion of the wire (see figure~\ref{Fig:Surf_Lin_melt}). 

\begin{figure}[htp]
	\centering
{\includegraphics[width=0.45\textwidth]{Figures/Surf_Lin_melt}}
    \caption{A surface melted nanowire of radius $R$ and length $H$ now with a liquid gap $h$. The solid core radii and length is $r$ and $H-h$ respectively. The solid and liquid phases are indicated as before.}
	\label{Fig:Surf_Lin_melt}   
\end{figure}

As before we write the free energy in terms of the free energy of the bulk (the volume) and the surface of the solid and liquid components:
\begin{equation}
\begin{split}
& F(r,h) = -\pi r^2(H-h)\rho L(1-T/T_c) + \pi R^2Hf_l  \\ 
& + 2 \pi RH\gamma_{lv} + 2 \pi r(H-h)(\gamma_{sl} + \Delta \gamma e^{-(R-r)/\xi}) \\ 
& + 2 \pi r^2 \gamma_{sl}(1-e^{-h/\xi})
\label{eqn:Fsurf_lin2}
\end{split}
\end{equation}
Note the introduction of thickness dependent solid-liquid interfacial energy $\gamma_{sl}(1-e^{-h/\xi})$ that represents the interaction of the two solid-liquid interfaces across the break in the wire. Note that as $h \rightarrow 0$, the energy $2 \pi r^2 \gamma_{sl}(1-e^{-h/\xi}) \rightarrow 0$. 

It is straightforward to show that for $r=R$, the free energy $F(r,h)$ does not exhibit a minima at $h=0$ i.e. $\left. \partial F/\partial h \right|_{r=R} \neq 0$. a To find minima in this we need to solve for $\partial F/\partial r = \partial F/\partial h = 0$ simultaneously.

% \begin{flushleft}
% \begin{equation}
% \begin{split}
% & \frac{\partial F}{\partial r} = -2\pi r(H-h)\rho L(1-T/T_c) + 4\pi r \gamma_{sl}(1-e^{-h/\xi}) \\ 
% & + 2\pi (H-h)(\gamma_{sl} + \Delta \gamma(1 + r/\xi)e^{-(R-r)/\xi}) = 0
% \label{eqn:dFdr}
% \end{split}
% \end{equation}

% \begin{equation}
% \begin{split}
% & \frac{\partial F}{\partial h} = \pi r^2\rho L(1-T/T_c) + \frac{2\pi r^2 \gamma_{sl}}{\xi}e^{-h/\xi} \\ 
% & - 2\pi r(\gamma_{sl} + \Delta \gamma e^{-(R-r)/\xi}) = 0
% \label{eqn:dFdh}
% \end{split}
% \end{equation}
% \end{flushleft}

To find these minima, surface plots of \cref{eqn:Fsurf_lin2} with respect to the solid were computed (\textit{i.e. the 2nd and 3rd terms in \cref{eqn:Fsurf_lin2} were omitted}). The model showed that for $r=R$ and $h=0$ at $T = T_s$ a global minima was found. Then along the $h=0$ curve as $T \rightarrow T_m$ the global minima shifted to $r=0$ which is to be expected. Beyond this the only situation for $r\leq R$ and $T \rightarrow T_m$ where global minima found were for the $h = 0$ curve. 
\\
\textcolor{red}{This indicative that surface (radial) melting is a second-order transition, but the linear melting process is first-order.} \textcolor{blue}{Consider revising.}

% Using the literate values from Table I, \cref{eqn:Fsurf_lin2} was computed. Surface plots of \cref{eqn:Fsurf_lin2} at $T_s$ and $T_m$ we can see that along the $h = 0$ curve(s) there is a clear preference for surface melting and complete melting respectively.


\begin{figure*}[htp]
\centering
  \subfloat[FES of Ni at $T=T_s$. The FES clearly doesn't yield any minima (or maxima) as $h/H \rightarrow 1$. The only plausible solutions are for $h/H \rightarrow 0.$]{
  \includegraphics[width=.43\textwidth]{Figures/Ni_FES_T_1391}}
    \label{fig:FES_Ts}
  \subfloat[FES of Ni at $T=T_m$, where the minimum has shifted from the surface at $r=R$ to the center at $r=0$.]{
  \includegraphics[width=.43\textwidth]{Figures/Ni_FES_T_1430}}
    \label{fig:FES_Tm}
     \caption{This FES is for nickel a nickel nanowire with $R=10a$, $H=60a$ for $T \approx T_s$ and $T \approx T_m$ for $a)$ and $b)$ respectively. As we increase $T_s \rightarrow T_m$ the global minima at shifts away from $r=R$ and moves toward $r=0$.}
     \label{Fig:Ni_FES}
\end{figure*}

\vspace{0.5cm}


%\begin{figure*}
%\centering
%\begin{minipage}[htp]{.30\textwidth}
%  \includegraphics[width=1.05\linewidth]{Figures/FreeEngXZ_R8_1350}
%  \label{fig:FESXZ_Ts}
%  \caption{Projection of \Cref{fig:FES_Ts} onto the XZ plane for $T=T_s$}
%\end{minipage}\qquad
%\begin{minipage}[htp]{.30\textwidth}
%  \includegraphics[width=1.05\linewidth]{Figures/FreeEngXZ_R8_1355}
%  \label{fig:FESXZ_T}
%  \caption{Projection of Ni FES onto the XZ plane for $T_s<T<T_m$}
%\end{minipage}\qquad
%\begin{minipage}[htp]{.30\textwidth}
%  \includegraphics[width=1.05\linewidth]{Figures/FreeEngXZ_R8_1358}
%  \caption{Projection of \Cref{fig:FES_Tm} onto the XZ plane for $T=T_m $}
%  \label{fig:FESXZ_Tm}
%\end{minipage}
%\end{figure*}

\begin{figure*}[htp]
\centering
  \subfloat[Projection of \Cref{Fig:Ni_FES} \textbf{$a)$} onto the XZ plane for $T \approx T_s$]{
  \includegraphics[width=.32\textwidth]{Figures/Ni_Fsur_T_1378}}
    \label{fig:FESXZ_Ts}
  \subfloat[Projection of Ni FES onto the XZ plane for $T_s<T<T_m$]{
  \includegraphics[width=.32\textwidth]{Figures/Ni_Fsur_T_1396}}
  \label{fig:FESXZ_T}
  \subfloat[Projection of \Cref{Fig:Ni_FES} \textbf{$b)$} onto the XZ plane for $T \approx T_m$]{
  \includegraphics[width=.32\textwidth]{Figures/Ni_Fsur_T_1417}}
   \label{fig:FESXZ_Tm}
     \caption{The projects on the nickel FES onto the XZ plane gives perspective on how the global minima begins to shift as we increase in $T$. We can see that as $T > T_m$ that the $F(r,h) > 0$ which is an indicator that the wire is completely liquid.}
     \label{Fig:Ni_FES_XZ}
\end{figure*}


%
%\begin{figure*}[htp]
%\centering
%  \subfloat[FES of Ni at $T=T_s$. The FES clearly doesn't yield any minima or maxima for that matter as $h/R \rightarrow H/R$, and the only plausible solutions are for $h/R \rightarrow 0.$]{
%  \includegraphics[width=.90\textwidth]{Figures/Free_Eng_Al_R10}}
%    \label{fig:FES_Al}
%\end{figure*}


\begin{figure*}[htp]
\centering
  \subfloat[Projection of the aluminium FES onto the XZ plane for some $T_i<T_m$]{
  \includegraphics[width=.32\textwidth]{Figures/Al_Fsur_T_819}}
  \label{fig:FESALXZ_Ti}
  \subfloat[Projection of the aluminium FES onto the XZ plane for $T_i<T<T_m$]{
  \includegraphics[width=.32\textwidth]{Figures/Al_Fsur_T_825}}
  \label{fig:FESALXZ_T}
  \subfloat[Projection of the aluminium FES onto the XZ plane for $T=T_m $]{
  \includegraphics[width=.32\textwidth]{Figures/Al_Fsur_T_829}}
  \label{fig:FESALXZ_Tm}
     \caption{The projection of the aluminium FES onto the XZ plane behaves quite differently than it does for \cref{Fig:Ni_FES_XZ}. As $T_m$ is approached, the global minimum shifts abruptly from $r=R$ to $r=0$, and doesn't transition away like what it does for nickel.}
     \label{Fig:Al_FES_XZ}
\end{figure*}



%\begin{figure*}
%\centering
%\begin{minipage}[htp]{.30\textwidth}
%  \includegraphics[width=1.05\linewidth]{Figures/Al_Fsur_T_819}
%  \label{fig:FESALXZ_T}
%  \caption{Projection of the aluminium FES onto the XZ plane for some $T_i<T_m$}
%\end{minipage}\qquad
%\begin{minipage}[htp]{.30\textwidth}
%  \includegraphics[width=1.05\linewidth]{Figures/Al_Fsur_T_825}
%  \label{fig:FESALXZ_T}
%  \caption{Projection of the aluminium FES onto the XZ plane for $T_i<T<T_m$}
%\end{minipage}\qquad
%\begin{minipage}[htp]{.30\textwidth}
%  \includegraphics[width=1.05\linewidth]{Figures/Al_Fsur_T_829}
%  \caption{Projection of the aluminium FES onto the XZ plane for $T=T_m$}
%  \label{fig:FESALXZ_Tm}
%\end{minipage}
%\end{figure*}

Using the literate values from Table I, \cref{eqn:Fsurf_lin2} was computed. Surface plots of \cref{eqn:Fsurf_lin2} at $T_s$ and $T_m$ we can see that along the $h = 0$ curve(s) there is a clear preference for surface melting and complete melting respectively.

Looking at the projections of the FES onto the XZ plane we can see that the global minima shifts from being at $r=R$ at $T=T_s$ to $r=0$ at $T=T_m$. As before mentioned there is a clear preference for surface melting or complete melting. For $T_s < T < T_m$ there is only a global minima along the $h=0$ line which infers that a surface melted wire with the presence of a liquid gap is not a stable state. As $T_s \rightarrow T_m$ the global minima shifts from $r=R$ to $0<r<R$ to $r=0$ which is indicative that there are stable surface melted states that exist between $T_s$ and $T_m$. For aluminium the nature of the FES is different. Firstly since we have calculated $\Delta \gamma < 0$ from the literature values obtained, \cref{eqn:Tsurf} implies that $T_s > T_m$. As seen in the previous section, this doesn't agree with the simulated data. At some temperature $T_i < T_m$ the global minima sits at the $h=0$ curve at $r=R$. As $T_i \rightarrow T_m$ the location of the global minima only shifts away from $r=R$ to $r=0$ once $T=T_m$ in contrast to what nickel demonstrates. \textcolor{red}{The conclusion from this was that the type of melting dynamics that aluminium experiences is far more \textit{discontinuous} type of phase transition whereas nickel is more \textit{continuous}, as we seen \cref{S:Sim_Res} in the simulated results section. Additionally this result is plausible from what other computational and theoretical studies have shown \cite{hendy2009superheating, schebarchov2006superheating} in that aluminium can remain solid up until it reaches its melting temperature.} \textcolor{blue}{Consider revising. Want references or some more solid points as to how the nature of the FES' imply that surface melting is continuous and linear melting is discontinuous.}


==> Old_model.tex <==
Such models have been investigated extensively for spherical geometries \cite{hendy2010superheating} in order to understand these phenomena in nanoparticles, and have been tested in experiments on the melting of supported particles \cite{lai1996size}. Melting occurs when the free energies of the solid and liquid state are equal (\textit{i.e.} when $F_s = F_l$). Here we assume that the cylindrical structure remains stable, and no break up of the wire (or the solid core) occurs. 

We consider the free energy difference between a length $H$ of (an infinitely long) cylindrically symmetric solid of radius $R$ and the corresponding molten cylinder:
\begin{equation}
	\Delta F = F_s - F_l = \pi R^2H(f_s - f_l) + 2\pi RH(\gamma_{sv} - \gamma_{lv})
\end{equation}
where $f_s$ and $f_l$ are the free energy densities of the solid and liquid respectively. Using the relation $f_l - f_s = \rho L \left( 1 - T/T_c\right)$
(where $\rho$ is the density, $L$ is the latent heat of melting, and $T_c$ is the bulk melting temperature), the melting temperature $T_m$ (i.e. the temperature at which $\Delta F = 0$) is found to be
\begin{equation}
	T_m = T_c\left(1-\frac{2(\gamma_{sv}-\gamma_{lv})}{\rho LR} \right),
    \label{eqn:Tmelt}
\end{equation}
illustrating the familiar result that the melting point of a wire is inversely proportional to the wire radius.

To describe surface melting, we need to consider the free energy of a surface melted wire (see Fig.~\ref{Fig:Surf_melt}) with solid core of radius $r$. The free energy can be expressed as a function of $r$
as follows\begin{equation}
\begin{split}
F(r) = \pi(R^2 - r^2)Hf_l	 + \pi r^2 Hf_s + 2 \pi RH\gamma_{lv} &\\ + 2 \pi rH(\gamma_{sl} + \Delta \gamma e^{-(R-r)/\xi}).
\label{eqn:Fsurf}
\end{split}
\end{equation}
The term last term $\Delta \gamma e^{(R-r)/\xi}$ models the interaction between the liquid-vapour and solid-liquid interface, which decays exponentially with a correlation length $\xi$ $\cite{van1990ion}$. For a surface melted Al (111), for example, $\xi$ has been estimated to be 3 \AA \cite{di1995maximum, pluis1990surface}. Note that this term ensures that as $r \rightarrow R$, $F(r) \rightarrow F_s$ (the free energy of a solid cylinder of radius $R$), and that as $r \rightarrow 0$, $F(r) \rightarrow F_l$ (the free energy of a liquid cylinder of radius $R$). 

The onset of surface melting may occur at the temperature $T_s$ at which a minimum in the free energy $F(r)$ appears at $r=R$:
\begin{equation}
T_{s} = T_c\left[1 - \frac{\gamma_{sv}-\gamma_{lv}}{\rho LR}\left(1 + \frac{R}{R_{c}}\right) \right]
\label{eqn:Tsurf}
\end{equation}
where $R_{c} = \frac{\gamma_{sv}-\gamma_{lv}}{\Delta\gamma}\xi$.
